Fair Allocation with Interval Scheduling Constraints

We study a fair resource scheduling problem, where a set of interval jobs are to be allocated to heterogeneous machines controlled by agents. Each job is associated with release time, deadline, and processing time such that it can be processed if its complete processing period is between its release time and deadline. The machines gain possibly different utilities by processing different jobs, and all jobs assigned to the same machine should be processed without overlap. We consider two widely studied solution concepts, namely, maximin share fairness and envy-freeness. For both criteria, we discuss the extent to which fair allocations exist and present constant approximation algorithms for various settings.

==> 05-others.tex <==
\section{More Stories}

In this work, we initiated the work of fair division of intervals. 
Our target is to investigate whether fairness and efficiency can be guaranteed simultaneously. 
As shown by our theorems, in general PO and IO are not compatible with EF1. However, this are special yet typical and commonly-seen cases where we are able to compute an allocation that is both EF1 and PO/IO. 
For example, in \cref{thm:EF1+PO:weighted:p}, we have proved that when agents have arbitrary utilities and all jobs have unit processing time, we able to find an allocation that is EF1 and PO. An interesting question is if this result can be extended to the case when agents have weighted or even matrix weighted.
In this section, we first answer this question regarding weighted utilities affirmatively and then show some evidences for matrix utilities. 

% \subsection{Weighted Utilities}
% \begin{theorem}\label{thm:EF1+PO:weighted}
% There is an allocation that is simultaneously EF1 and PO if agents have weighted utilities and all jobs have unit processing time.
% \end{theorem}

% Before we prove the \cref{thm:EF1+PO:weighted}, we first provide the following notations. We also use the maximum matching-based algorithm. We use the same bipartite graph construction method as \cref{alg:cardinality:p_j=1:EF1}. Since we consider the weighted utilities functions in this section, each edge in $G(\cJ,\cT)$ is additionally associated with a weight, i.e.,
% % Given an arbitrary instance of \FISP/ with unit processing jobs and weighted weigh, for each job $j_i\in\mathcal{J}$, let $\mathcal{T}_i$ be the set of time slots included in the job window of $j_i$, i.e., $\mathcal{T}_i=\set{r_i,r_i+1,\cdots,d_i}$. Let $\mathcal{T}=\bigcup_{1\leqslant i \leqslant n}\mathcal{T}_i$. Note that the size of $\mathcal{T}$ can eb bounded by $O(n^2)$, where $n$ is the number of jobs. For each time slot $t_o\in\mathcal{T}$, we create $m$ copies, i.e., let $t_l^r$ be the $l$-th time slot in the $r$-th machine (agents), where $1\leqslant r \leqslant m$. Let $\mathcal{T}^M$ be the constructed time slot set. Note that the size of $\mathcal{T}^M$ can be bounded by $O(mn^2)$. Now we are ready to construct a weighted bipartite graph $G(X\cup Y, E)$. For each job $j\in\mathcal{J}$, we have one vertex in $X$. For each time slot $t\in\mathcal{T}^M$, we have one vertex in $Y$. $E$ has an edge between a job vertex $x_i\in X$ and every time slot vertex in $\set{t_l^r|1\leqslant r \leqslant m}\subseteq\mathcal{T}^M$ if and only if $t_l\in\mathcal{T}_i$. 
% every edge in $\set{(j_i,t_l^r)\in E|t_l\in\mathcal{T}_i,1\leqslant r \leqslant m}$ has the same weight $w_i$, where $w_i$ is the weight for job $j_i$. Let $M$ be an arbitrary maximum weighted matching in bipartite graph $G(\mathcal{J},\mathcal{T})$. Let $M(J)$ and $M(T)$ be the set of job vertices and time slot vertices in $M$, respectively. Let $\mathcal{J}_M$ be the set of job whose corresponding job vertex is in $M(J)$. Let $M_i\subseteq M$ be the set of (job,time slot) pairs whose time slot vertex in $i$-th machine (agent), where $1\leqslant i \leqslant m$, i.e., $M_i=\set{(j,t_l^r)\in M|r=i}$. Note that $\mathcal{M}=\set{M_1,M_2,\cdots,M_m}$ is a partition to $M$. Let $M_i(J)$ and $M_i(T)$ be the set of job vertices and time slot vertices included in matching $M_i$, respectively. Note that $\mathcal{M}(J)=\set{M_1(J),M_2(J),\cdots,M_m(J)}$ and $\mathcal{M}(T)=\set{M_1(T),M_2(T),\cdots,M_m(T)}$ is the partition to $M(J)$ and $M(T)$, respectively. Note that $|M_i|=|M_i(J)|,\forall 1\leqslant i \leqslant m$. Let $M_i\in\mathcal{M}$ be an arbitrary matching, for each time slot $t_k^i\in\mathcal{T}^M$, we define $g_k^i$ as the \textit{price} of time slot $t_k^i$, i.e., 
% $$
% g_k^i=
% \begin{cases}
% w_l, & \exists (j_l,t_k^i)\in M_i.\\
% 0, & \text{otherwise}.\\
% \end{cases}
% $$

% \begin{algorithm}[htb]
% \caption{\hspace{-2pt}{\bf .} Maximum matching-based algorithm for $p_j=1$ and arbitrary weight}
% \label{alg:weight:p_j=1:EF1}
% \begin{algorithmic}[1]
% \REQUIRE $\mathcal{M}=\set{M_1,M_2,\cdots,M_m}$.
% \ENSURE EF1 allocation $\mathcal{X}= (X_0, X_1, \cdots ,X_m)$.
% \STATE $X_0=\mathcal{J}-\mathcal{J}_M$.
% \WHILE{there is two matchings $M_i,M_k\in\mathcal{M}$ such that $\sum_{j_l\in M_i(J)}w_l-\max_{j_l\in M_i(J)}\{w_l\} > \sum_{j_o\in M_k(J)}w_o$}
% \label{line:weight:2}

% \WHILE{$\sum_{j_l\in M_i(J)}w_l-\max_{j_l\in M_i(J)}\{w_l\} > \sum_{j_o\in M_k(J)}w_o$}
% \label{line:weight:3}
%     \STATE $t_a^i,t_a^k=\argmax\limits_{t_b^i\in M_i(T),t_b^i\in M_k(T)}\{\frac{g_b^i}{g_b^k}\}$.
%     \label{line:weight:4}
%     \STATE Find $(j,t_a^i)\in M_i$ and $(j',t_a^k)\in M_k$.
%     \STATE $M_i=M_i\cup\set{(j',t_a^i)}\setminus\set{(j,t_a^i)}$. 
%     \STATE $M_k=M_k\cup\set{(j,t_a^k)}\setminus\set{(j',t_a^k)}$.
%     \label{line:weight:7}
% \ENDWHILE
% \label{line:weight:8}

% \ENDWHILE
% \label{line:weight:9}

% \FOR{$1\leqslant i \leqslant m$}
%     \STATE $X_i:=M_i(J)$.
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

% Let $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$ be the allocation returned by \cref{alg:weight:p_j=1:EF1}.

% \begin{observation}
% The allocation $\cX$ maximizes social welfare, i.e., there is no another feasible allocation $\cX'=\set{X_0,'X_1',\cdots,X_m'}$ such that $\sum_{i=1}^{m}u(X_i')>\sum_{i=1}^{m}u(X_i)$.
% \label{obs:weighted:p_j=1:EF1:PO}
% \end{observation}

% \begin{lemma}
% $u_i(X_i)\geqslant u_i(X_0\cup X_i),\forall 1\leqslant i \leqslant m$.
% \label{lem:weight:p_j=1:EF1:charity}
% \end{lemma}

% \begin{proof}
% We prove by contradiction and therefore assume that there exists an agent $a_i\in\mathcal{A}$ such that $u_i(X_i) < u_i(X_0\cup X_i)$. We prove by constructing two weighted bipartite graphs, denoted by $G(X_i,\mathcal{T}^1)$ and $G(X_0\cup X_i,\mathcal{T}^1)$. In $G(X_i,\mathcal{T}^1)$, we have $|X_i|$ vertices in one side, one vertex for one job in $X_i$, we have $|\mathcal{T}|$ vertices in another side, one vertex for one time slot in $\mathcal{T}$. There is an edge between job vertex and time slot vertex if and only if the time slot is in the job window. Each edge in $\set{(j_i,t)\in|j_i=j_i'}$ has the same weight $w_i$, In $G(X_0\cup X_i,\mathcal{T}^1)$, we have $|X_0\cup X_i|$ vertices in one side, one vertex for one job in $X_0\cup X_i$, and the remaining part is similar as the $G(X_i,\mathcal{T}^1)$. Let $M_i,M_i'$ be the maximum weighted matching in $G(X_i,\mathcal{T}^1),G(X_0\cup X_i,\mathcal{T}^1)$, respectively. Let $v(M_i),v(M_i')$ be the value of maximum weighted matching $M_i,M_i'$, respectively. Observe that $u_i(X_i)=\sum_{j_l\in X_i}w_l=v(M_i)$ and $u_i(X_0\cup X_i)=\sum_{j_l\in X_0\cup X_i} w_l=v(M_i')$. Since $u_i(X_i)<u_i(X_0\cup X_i)$, we have $v(M_i)<v(M_i')$. Since the partition $\mathcal{M}=\set{M_1,\cdots,M_m}$ of the maximum weighted matching in $G(\mathcal{J},\mathcal{T})$ corresponds to the allocation $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$ returned by \cref{alg:weight:p_j=1:EF1}, we construct a new partition, denoted by $\mathcal{M}'$, in the following ways: $\mathcal{M}'=\mathcal{M}\cup\set{M_i'}\setminus\set{M_i}$. It is easy to see $\mathcal{M}'$ is a matching in $G(\mathcal{J},\mathcal{T})$. Since $v(M_i)<v(M_i')$, we have $v(\mathcal{M}')=\sum_{M_i\in\mathcal{M}'}v(M_i) > v(\mathcal{M})=\sum_{M_i\in\mathcal{M}}v(M_i)$. This implies that $M$ is not the maximum matching in $G(\mathcal{J},\mathcal{T})$ which contradicts our assumption.
% \end{proof}

% \begin{lemma}
% $u_i(X_i)\geqslant u_i(X_k\setminus\set{j}),\forall i\in[m]$ and $\exists j\in X_k$.
% \label{lem:weight:p_j=1:EF1:agents}
% \end{lemma}

% \begin{proof}
% It is easy to see the correctness of \cref{lem:weight:p_j=1:EF1:agents}. \cref{alg:weight:p_j=1:EF1} stops at the case where there is no $X_i,X_k\in\mathcal{X}$ such that $\sum_{j_l\in X_i}w_l - \max_{j_l\in X_i}\{w_l\} > \sum_{j_o\in X_k}w_o$.
% \end{proof}

% Let $M_i\in\mathcal{M}$ and $M_k\in\mathcal{M}$ be two matchings such that $\sum_{j_l\in M_i(J)}w_l-\max_{j_l\in M_i(J)}\{w_l\} > \sum_{j_o\in M_k(J)}w_o$. Let $M_i'$ and $M_k'$ be two matchings generated from $M_i$ and $M_k$ by running Line \ref{line:weight:3}-\ref{line:weight:8} of \cref{alg:weight:p_j=1:EF1}. We define $v(M_i)=\sum_{j_l\in M_i(J)}w_l$ for convenience. Similar definitions for $v(M_k),v(M_i'),v(M_k')$. Since $v(M_i)-\max_{j_l\in M_i(J)}\{w_l\}>v(M_k)$, we have $v(M_i)>v(M_k)$.

% \begin{lemma}
% The following four inequalities hold:
% \begin{enumerate}
%     \item $v(M_i)>v(M_i')$;
%     \item $v(M_i)>v(M_k')$;
%     \item $v(M_k)<v(M_i')$;
%     \item $v(M_k)<v(M_k')$.
% \end{enumerate}
% \label{lem:weighted:p_j=1:EF1:running_time:key}
% \end{lemma}

% \begin{proof}
% We consider an arbitrary time's while loop (line \ref{line:weight:3}-\ref{line:weight:8} of \cref{alg:weight:p_j=1:EF1}). Observe that $\max\limits_{t_b^i\in M_i(T),t_b^i\in M_k(T)}\{\frac{g_b^i}{g_b^k}\}>1$, otherwise it is impossible that $v(M_i)>v(M_k)$. Let $t_a^i,t_a^k=\argmax\limits_{t_b^i\in M_i(T),t_b^i\in M_k(T)}\{\frac{g_b^i}{g_b^k}\}$. Assume that job $j,j'$ is matched with time slot $t_a^i,t_a^k$, respectively, i.e., $(j,t_a^i)\in M_i,(j',t_a^k)\in M_k$.  In every such while loop, we exchange the job $j$ with $j'$, i.e., $M_i(J)=M_i(J)\cup\set{j'}\setminus\set{j}$ and $M_k(J)=M_k(J)\cup\set{j}\setminus\set{j'}$. Since $\frac{g_a^i}{g_a^k}>1$, we have $v(M_i)>v(M_i')$ and $v(M_k)<v(M_k')$ which implies that the first and fourth inequality holds.

% Now, we still consider an arbitrary time's while loop (line \ref{line:weight:3}-\ref{line:weight:8} of \cref{alg:weight:p_j=1:EF1}). The while loop does not stop because of $v(M_i)-\max_{j_l\in M_i(J)}\{w_l\}>v(M_k)$. \cref{alg:weight:p_j=1:EF1} will exchange two jobs in Line \ref{line:weight:4}-\ref{line:weight:7}. Let $j_o\in M_i(J),j_o'\in M_k(J)$ and assume that \cref{alg:weight:p_j=1:EF1} exchange $j_o$ with $j_o'$ in this time's while loop (line \ref{line:weight:3}-\ref{line:weight:8} of \cref{alg:weight:p_j=1:EF1}). Let $M_i'',M_k''$ be the resulting matching after exchanging. We have $v(M_i'')=v(M_i)-w_o+w_{o}'$ and $v(M_k'')=v(M_k)-w_o'+w_o$. Observe that $v(M_i)-v(M_k'')=v(M_i)-v(M_k)-w_o+w_o'$. Since $v(M_i)-\max_{j_l\in M_i(J)}\{w_l\}>v(M_k)$ and $\max_{j_l\in M_i(J)}\{w_l\}>w_o$, we have $v(M_i)-v(M_k'')>0$ which implies that the second inequality holds. Observe that $v(M_i'')-v(M_k)=v(M_i)-v(M_k)-w_o+w_o'=v(M_i)-v(M_k'')$, we have $v(M_i'')-v(M_k)>0$ which implies that third inequality holds.
% \end{proof}

% % \begin{theorem}
% % There is an allocation that is simultaneously EF1 and PO if agents have weighted utilities and all jobs have unit processing time.
% % \end{theorem}

% Now we are ready to prove \cref{thm:EF1+PO:weighted}.

% \begin{proof}[Proof of \cref{thm:EF1+PO:weighted}]
% % According to \cref{lem:weight:p_j=1:EF1:charity} and \cref{lem:weight:p_j=1:EF1:agents}, \cref{alg:weight:p_j=1:EF1} will return an EF1 allocation. 

% According to \cref{obs:weighted:p_j=1:EF1:PO}, we know that the feasible allocation $\cX$ returned by \cref{alg:weight:p_j=1:EF1} maximizes the social welfare. Therefore, $\cX$ is a PO allocation. According to \cref{lem:weight:p_j=1:EF1:agents}, we know that $\cX$ is an EF1 allocation. Hence, \cref{alg:weight:p_j=1:EF1} will return a feasible allocation that is simultaneously EF1 and PO.

% Now, we prove the running time. We consider an arbitrary iteration of line \ref{line:weight:2}-\ref{line:weight:9} of \cref{alg:weight:p_j=1:EF1}. The four inequalities in \cref{lem:weighted:p_j=1:EF1:running_time:key} imply that, after every time's while loop (line \ref{line:weight:2}-\ref{line:weight:9} of \cref{alg:weight:p_j=1:EF1}), the value of two generated matchings will be strictly between the value of two old matchings, i.e., $v(M_i)>v(M_i'),v(M_k')>v(M_k)$. In every while loop (line \ref{line:weight:2}-\ref{line:weight:9} of \cref{alg:weight:p_j=1:EF1}), the value of $M_k$ will be increased strictly. Note that in the following's while loop (line \ref{line:weight:2}-\ref{line:weight:9} of \cref{alg:weight:p_j=1:EF1}), the value of $v(M_k')$ may be decreased again, but the value of new $v(M_k')$ will never be smaller than the value of old $v(M_k')$. To prove the running time of \cref{alg:weight:p_j=1:EF1}, we implement \cref{alg:weight:p_j=1:EF1} by always choosing the matching with the minimum value of $v(\cdot)$, i.e., $M_k=\min_{M_l\in\cM}\{v(M_l)\}$. After one while loop (line \ref{line:weight:2}-\ref{line:weight:9} of \cref{alg:weight:p_j=1:EF1}), we know that $v(M_k)$ will be increased strictly but it does not imply that $\min_{M_l\in\cM}\{v(M_l)\}$ is also increased because there may exist many agents share the minimum value of $v(\cdot)$. But it is easy to see that after $m$ times' while loop (line \ref{line:weight:2}-\ref{line:weight:9} of \cref{alg:weight:p_j=1:EF1}), the value of  $\min_{M_l\in\cM}\{v(M_l)\}$ must be increased, where $m$ is the number of agents.

% Let $\cW=\set{w_1,w_2,\cdots,w_n}$ be the set of weights of all jobs in $\cJ$. To describe the increase in the minimum value of $v(\cdot)$, we assume that every weight in $\cW$ is an integer otherwise we can scale all weights. According the above proof, we know that after $m$ iterations, the overall minimum value of $v(\cdot)$ must be increased. Since all weights are integral, the increase is at least $1$. Hence, the while loop in line \ref{line:weight:2}-\ref{line:weight:9} of \cref{alg:weight:p_j=1:EF1} will be run at most $m\cdot H$ times, where $m$ is the number of agents and $H=\sum_{w_i\in\cW}w_i$ is the summation of all the weight. Finding the maximum weighted matching requires $O((n+mn^2)^2(mn^3))=O(m^3n^7)$. Running line \ref{line:weight:3}-\ref{line:weight:8} takes $O(n)$ time. We have running time: $O(m^3n^7+mn\cdot H)$, where $n$ is the number of jobs, $m$ is the number of agents and $H=\sum_{w_i\in\cW}w_i$.

% % (\ruilong{pseudo-polynomial time!!! It's okay})
% % \bo{Awesome!}
% \end{proof}
\subsection{Cardinality Utilities and arbitrary processing time}


\subsection{Matrix Utilities and unit processing time}



==> 91-ef.tex <==
\section{Existence and hardness for EF allocation}

Let us show a job system may not have \textit{EF}, even in the case where each job has an unit processing time and a  cardinality weight. We prove by giving an instance. See  \cref{exa:no_ef}.

\begin{example}
Consider a job system including an agent set $\mathcal{A}$ with size $m$ and a job set $\mathcal{J}$ with the size $n=m+1$, i.e., $|\mathcal{J}|=|\mathcal{A}|+1$. Each job has an unit processing time and cardinality weight, i.e., $\forall j\in\mathcal{J},p_j=1$, and $w_{ij}=1,\forall i\in[m],j\in[n]$. Moreover, each job has an unique time slot to process, i.e., $\forall j\in\mathcal{J},r_j=d_j$ and $\forall j,j'\in\mathcal{J},r_j\ne r_{j'}$.
\label{exa:no_ef}
\end{example}

\begin{lemma}
There is no feasible allocation $\mathcal{X}$ such that  $\mathcal{X}$ is an \textit{EF} allocation in \cref{exa:no_ef}.
\end{lemma}

\begin{proof}
We consider an arbitrary feasible allocation $\mathcal{X}=(X_0,X_1,\cdots,X_m)$. Suppose that $X_0\ne\emptyset$. We can consider an arbitrary agent $a_i\in\mathcal{A}$. Then, we have $u_{i}(X_i)<u_{i}(X_i\cup X_0)$ since each job has an unique time slot to process. Hence, $\mathcal{X}$ is not an EF allocation. Therefore, we assume that $X_0=\emptyset$, otherwise $\mathcal{X}$ must not be an EF allocation. According to the pigeonhole principle, $n=m+1$ jobs are assigned to $m$ agents, then at least one agent, denoted by $a_i$, receives at least $\lfloor (n-1)/m \rfloor + 1 =2$ jobs, i.e., $|X_i|\geqslant 2$. Note that at least one agent, denoted by $a_j$, receives $0$ or $1$ job, otherwise the total number of jobs would be at least $2\cdot m$. Then, we have $u_{j}(X_i)=|X_i|>u_{j}(X_j)=|X_j|$ which implies that $\mathcal{X}$ is not an EF allocation. Thus, there is no EF allocation in \cref{exa:no_ef}.
\end{proof}

\begin{theorem}
Given an arbitrary instance of \FISP/, the EF allocation does not exist, even in the case where each job has an unit processing time and cardinality weight.
\end{theorem}

% Now, we know the existence of the EF allocation. Then, given an arbitrary instance of \FISP/, we consider the hardness of determining whether it has an EF allocation or not.

% \ruilong{determine whether there is an EF allocation for the problem [1,1] should be ploynomially solvable.}

% We first consider the hardness of finding an EF allocation in the easiest case in which each job has an unit processing time and cardinality weight. In the reminder of this paper, we denote this case by \FISP/ with unit processing time jobs and cardinality weight, i.e., $\forall j\in\mathcal{J},p_j=1$ and $w_{ij}=1,\forall i\in[m],j\in[n]$.

% Given an arbitrary instance of \FISP/ with unit processing time jobs and cardinality weight, for each job $j_i\in\mathcal{J}$, let $\mathcal{T}_i$ be the set of time slots included in the job window of $j_i$, i.e., $\mathcal{T}_i=\set{r_i,r_i+1,\cdots,d_i}$. Let $\mathcal{T}=\cup_{1\leqslant i \leqslant n}\mathcal{T}_i$. Note that the size of $\mathcal{T}$ can be bounded by $O(n^2)$, where $n$ is the number of jobs. For each each time slot $t_o\in\mathcal{T}$, we create $m$ copies, i.e., let $t_l^r$ be the $l$-th time slot in the $r$-th machine (agent), where $1\leqslant r \leqslant m$. Let $\mathcal{T}^M$ be the constructed time slot. Note that the size of $\mathcal{T}^M$ can be bounded by $O(mn^2)$. Now we are ready to construct a bipartite graph $G(X\cup Y,E)$. For each job $j\in\mathcal{J}$, we have one vertex in $X$. For each time slot $t\in\mathcal{T}^M$, we have one vertex in $Y$. $E$ has an edge between a job vertex $x_i\in X$ and every time slot vertex in $\set{t_l^r|1\leqslant r \leqslant m}\subseteq \mathcal{T}^M$ if and only if $t_l\in\mathcal{T}_i$. In the reminder of this section, we define $G(X\cup Y,E)$ as $G(\mathcal{J},\mathcal{T})$ for convenience. Let $M$ be an arbitrary maximum matching in bipartite graph $G(\mathcal{J},\mathcal{T})$. Let $M(J)$ and $M(T)$ be the set of job vertices and time slot vertices in $M$, respectively. Let $\mathcal{J}_M$ be set of jobs whose corresponding job vertex is in $M(J)$, i.e., a job is included in $\mathcal{J}_M$ if and only if the corresponding job vertex is included in $M(J)$. Let $M_i\subseteq M$ be the set of (job, time slot) pairs whose time slot vertex is in $i$-th machine (agent), $1\leqslant i \leqslant m$, i.e., $M_i=\set{(j,t_l^r)|r=i}$. Note that $\mathcal{M}=\set{M_1,M_2,\cdots,M_m}$ is a partition to $M$. Let $M_i(J)$ and $M_i(T)$ be the set of job vertices and time slot vertices included in matching $M_i$, respectively. Note that $M(J)=\set{M_1(J),M_2(J),\cdots,M_m(J)}$ and $M(T)=\set{M_1(T),M_2(T),\cdots,M_m(T)}$ is the partition to $M(J)$ and $M(T)$, respectively. Note that $|M_i|=|M_i(J)|=|M_i(T)|,\forall 1\leqslant i \leqslant m$.

% \begin{algorithm}[htb]
% \caption{\hspace{-2pt}{\bf .} Maximum matching-based algorithm for $p_j=1$ }
% \label{alg:cardinality:p_j=1:EF1}
% \begin{algorithmic}[1]
% \REQUIRE $\mathcal{M}=\set{M_1,M_2,\cdots,M_m}$.
% \ENSURE EF1 allocation $\mathcal{X}= (X_0, X_1, \cdots ,X_m)$.
% \STATE $X_0=\mathcal{J}-\mathcal{J}_M$.
% \WHILE{there is $M_i$ such that $|M_i|>\lceil \frac{|\mathcal{J}-\mathcal{J}_M|}{m} \rceil$ or $|M_i| < \lfloor  \frac{|\mathcal{J}-\mathcal{J}_M|}{m} \rfloor$}

% \IF{$|M_i|>\lceil \frac{|\mathcal{J}-\mathcal{J}_M|}{m} \rceil$}
%     \WHILE{$|M_i|>\lceil \frac{|\mathcal{J}-\mathcal{J}_M|}{m} \rceil$}
%         \STATE Find the $M_j=\min_{M_l\in\mathcal{M}}\{M_l\}$. 
%         \STATE Find a pair $(j,t_l^i)\in M_i$ such that $t_l^j\notin M_j(T)$.
%         \STATE $M_i=M_i-\set{(j,t_l^i)}$.
%         \STATE $M_j=M_j\cup\set{(j,t_l^j)}$.
%     \ENDWHILE
% \ELSE
%     \WHILE{$|M_i| < \lfloor  \frac{|\mathcal{J}-\mathcal{J}_M|}{m} \rfloor$}
%         \STATE Find the $M_j=\max_{M_l\in\mathcal{M}}\{M_l\}$.
%         \STATE Find a pair $(j,t_l^j)\in M_j$ such that $t_l^i\notin M_i(T)$.
%         \STATE $M_i=M_i\cup\set{(j,t_l^i)}$.
%         \STATE $M_j=M_j-\set{(j,t_l^j)}$.
%     \ENDWHILE
% \ENDIF

% \ENDWHILE

% \FOR{$1\leqslant i \leqslant m$}
%     \STATE $X_i:=M_i(J)$.
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}

% \begin{lemma}
% \cref{alg:cardinality:p_j=1:EF1} finds a feasible allocation $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$ with the maximum size of $\bigcup_{1\leqslant i \leqslant m}X_i$.
% \label{lem:card:p_j=1:EF:determine:key1}
% \end{lemma}

% \begin{proof}
% \cref{alg:cardinality:p_j=1:EF1} starts from a maximum matching which implies that the allocation $\mathcal{X}$ returned by \cref{alg:cardinality:p_j=1:EF1} must maximize the size of $\mathcal{J}-X_0$. Therefore, we only prove the correctness of \cref{alg:cardinality:p_j=1:EF1}.

% We first consider the case in which there is an $M_i$ such that $|M_i|>\lceil \frac{|\mathcal{J}-\mathcal{J}_M|}{m} \rceil$. In this case, $|M_j|\leqslant \lfloor  \frac{|\mathcal{J}-\mathcal{J}_M|}{m} \rfloor$, where $M_j=\min_{M_l\in\mathcal{M}}\{M_l\}$.

% We now consider the case in which there is an $M_i$ such that $|M_i| < \lfloor  \frac{|\mathcal{J}-\mathcal{J}_M|}{m} \rfloor$
% \end{proof}

% \begin{lemma}
% Given an arbitrary instance of \FISP/ with unit processing time jobs and cardinality weight, if a feasible allocation $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$ is an EF allocation, then $\mathcal{X}$ has the maximum size of $\bigcup_{1\leqslant i \leqslant m}X_i$.
% \label{lem:card:p_j=1:EF:determine:key2}
% \end{lemma}

% \begin{proof}
% We consider an arbitrary instance of \FISP/ with unit processing time jobs and cardinality weight, and assume that there exists an EF allocation $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$. We prove that $\mathcal{X}$ has the maximum size of $\bigcup_{1\leqslant i \leqslant m}X_i$. Let $f_l(\mathcal{J}')$ be the maximum number of jobs that can be feasibly scheduled in $l$ machines (agents) when the given job set is $\mathcal{J}'$, where $1\leqslant l \leqslant m,\mathcal{J}'\subseteq \mathcal{J}$. Note that $f_l(\mathcal{J}')$ can be computed by maximum matching in bipartite matching. To compute the $f_l(\mathcal{J}')$, we construct a bipartite graph $G_l(X\cup Y,E)$, for each job $j\in\mathcal{J}'$, we have one vertex in $X$, for each time slot $t\in\mathcal{T}$, we have $l$ vertices in $Y$. $E$ have an edge between a job vertex $x_i\in X$ and all of copies of time slot vertex $t\in Y$ if and only if $t\in\mathcal{T}_i$. In the reminder of this proof, we define $G_l(X\cup Y,E)$ as $G_l(\mathcal{J}',\mathcal{T}_l)$ for convenience. It is easy to see $f_l(\mathcal{J}')$ is the maximum matching in $G_l(\mathcal{J}',\mathcal{T}_l)$. Note that $f_m(\mathcal{J})=|M|$. Since $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$ is an EF allocation, we have $f_1(X_0\cup X_i) \leqslant f_1(X_i),\forall 1\leqslant i \leqslant m$. To prove \cref{lem:card:p_j=1:EF:determine:key2}, we need to show that $f_m(X_0\cup X_1\cdots\cup X_m) \leqslant f_1(X_1)+f_1(X_2)+\cdots+f_1(X_m)$. Observe that if we can prove $f_m(X_0\cup X_1\cdots\cup X_m) \leqslant f_1(X_0\cup X_1)+f_1(X_0\cup X_2) + \cdots +f_1(X_0\cup X_m)$, then the above inequality holds. Since $f_1(X_0\cup X_i) \leqslant f_1(X_i),\forall 1\leqslant i \leqslant m$, we have $f_1(X_0\cup X_i)=f_1(X_i),\forall 1\leqslant i\leqslant m,$ by the definition of $f_l(\mathcal{J}')$. Note that $f_1(X_0\cup X_i),f_1(X_i)$ is the maximum matching in $G_1(X_0\cup X_i,\mathcal{T}_1),G_1(X_1,\mathcal{T}_1)$, respectively. Since $f_1(X_0\cup X_i)=f_1(X_i)$, we assume that the maximum matching in $G_1(X_0\cup X_i,\mathcal{T}_1)$ and $G_1(X_i,\mathcal{T}_1)$ are exactly same. Let $M^i$ be the maximum matching in $G_1(X_0\cup X_i,\mathcal{T}_1)$. Note that $|M^i|=f_1(X_0\cup X_i)=f_1(X_i),\forall 1\leqslant i \leqslant m $. Let $\hat{\mathcal{M}}=\bigcup_{1\leqslant i \leqslant m}M^i$. Let $\hat{\mathcal{M}}(J),\hat{\mathcal{M}}(T)$ be the set of job vertices and time slot vertices included in $\hat{\mathcal{M}}$. Note that $\hat{\mathcal{M}}(J)=\bigcup_{1\leqslant i \leqslant m}X_i$ and $|\set{(j,t')\in\hat{\mathcal{M}}|t'=t}|\leqslant m$. Now we consider an arbitrary maximum matching $M$ in $G_m(\mathcal{J},\mathcal{T}_m)$. Note that $|M|=f_m(X_0\cup X_1\cdots\cup X_m)$ and $|\hat{\mathcal{M}}|=f_1(X_0\cup X_1)+f_1(X_0\cup X_2) + \cdots +f_1(X_0\cup X_m)$.

% We first prove that there must exist a maximum matching $M$ in $G_m(\mathcal{J},\mathcal{T}_m)$ such that $M$ is a $\bigcup_{1\leqslant i \leqslant m}X_i$-saturating matching. Note that $\hat{\mathcal{M}}$ can also be regarded as a matching in $G_m(\mathcal{J},\mathcal{T}_m)$. We start from an arbitrary maximum matching $M$. If $M$ is a $\hat{\mathcal{M}}(J)$-saturating matching, then we are done. If $M$ is not a $\hat{\mathcal{M}}(J)$-saturating matching, there must exist a job $j\in\bigcup_{1\leqslant i \leqslant m}X_i$ such that $j\notin M(J)$. We know that there must exist a pair $(j,t)\in\hat{\mathcal{M}}$ and $t\in M(T)$, otherwise $M$ is not the maximum matching. Assume that $t$ is matched with a job $j'$ in $M$, i.e., $(j',t)\in M$. Then, we just add $(j,t)$ to $M$ and remove $(j',t)$ from $M$, i.e., $M=M\cup\set{(j,t)}-\set{(j',t)}$. We repeat above process until there is no $j\in\hat{\mathcal{M}}(J)$ such that $j\notin M(J)$. Note that above process must stop at the case where $M$ is a $\hat{\mathcal{M}}(J)$-saturating matching since $\hat{\mathcal{M}}$ can be regarded as a matching in $G_m(\mathcal{J},\mathcal{T}_m)$.

% Now we are ready to prove the inequality $f_m(X_0\cup X_1\cdots\cup X_m) \leqslant f_1(X_0\cup X_1)+f_1(X_0\cup X_2) + \cdots +f_1(X_0\cup X_m)$. We prove by contradiction and therefore assume that $f_m(X_0\cup X_1\cdots\cup X_m) > f_1(X_0\cup X_1)+f_1(X_0\cup X_2) + \cdots +f_1(X_0\cup X_m)$. We consider an arbitrary maximum matching $M$ and assume that $M$ is a $\hat{\mathcal{M}}(J)$-saturating matching, otherwise we can modify it. Since $|M|>|\hat{\mathcal{M}}|$, there must exist a pair $(j_d,t_d)\in M$ such that $j_d\notin\hat{\mathcal{M}}(J)$ which implies that $j_d\in X_0$. Then, we consider an arbitrary $X_i,i\in[m]$. And we have $\set{(j,t)\in M|j\in X_i}\cup \set{(j_d,t_d)}$ is a feasible matching with the size $|X_i|+1$. This implies that there exist a matching in $G_1(X_0\cup X_i,\mathcal{T}_1)$ with the size $|X_i|+1$. Then, we have $f_1(X_0\cup X_i) > f_1(X_i)$ which implies that allocation $\mathcal{X}$ is not an EF allocation. 
% \end{proof}

% \begin{lemma}
% If \cref{alg:cardinality:p_j=1:EF1} returns an allocation $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$ which is not an EF allocation, then $\frac{|\mathcal{J}-X_0|}{m}$ is not an integer.
% \label{lem:card:p_j=1:EF:determine:key3}
% \end{lemma}

% \begin{lemma}
% Given an arbitrary instance of \FISP/ with unit processing time jobs and cardinality weight, there is an EF allocation if and only if \cref{alg:cardinality:p_j=1:EF1} returns an EF allocation.
% \end{lemma}

% \begin{proof}
% ($\Leftarrow$) This direction is strainghtforward. If \cref{alg:cardinality:p_j=1:EF1} can return an EF allocation, it implies that there is an EF allocation for the given instance.

% ($\Rightarrow$) To prove this direction, we prove the following argument: if \cref{alg:cardinality:p_j=1:EF1} returns a feasible allocation $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$ which is not an EF allocation, then there is no EF allocation exists. We prove by contradiction. Suppose that there is an EF allocation $\mathcal{X}'=\set{X_0',X_1',\cdots,X_m'}$. According to \cref{lem:card:p_j=1:EF:determine:key2}, we know that allocation $\mathcal{X}'$ has the maximum size of $\bigcup_{1\leqslant i \leqslant m}X_i$. According to \cref{lem:card:p_j=1:EF:determine:key1}, we know that allocation $\mathcal{X}$ also has the maximum size of $\bigcup_{1\leqslant i \leqslant m}X_i$. Then, we have $|\bigcup_{1\leqslant i \leqslant m}X_i|=|\bigcup_{1\leqslant i \leqslant m}X_i'|$. According to \cref{lem:card:p_j=1:EF:determine:key3} and our assumption that $\mathcal{X}$ is an EF allocation, we know that $\frac{|\mathcal{J}-X_0|}{m}=\frac{|\bigcup_{1\leqslant i \leqslant m }X_i|}{m}$ is not an integer which implies that $|\bigcup_{1\leqslant i \leqslant m}X_i'|$ is not an integer either. Since $\mathcal{X}'$ is an EF allocation, we have $\forall a_i\in\mathcal{A},X_j'\in\mathcal{X'},u_i(X_i')=|X_i'|\geqslant u_i(X_j')=|X_j'|$. This implies that $|X_i'|=|X_j'|,\forall X_i',X_j'\in(\mathcal{X}'-X_0')$. Since $X_i'\cap X_j'=\emptyset,\forall X_i',X_j'\in(\mathcal{X}'-X_0')$, we have $|\bigcup_{1\leqslant i \leqslant m}X_i'|=m\cdot |X_i'|,$ for an arbitrary $i\in[m]$. Since $|X_i|$, for an arbitrary $i\in[m]$, is an integer, we have $|\bigcup_{1\leqslant i \leqslant m}X_i'|$ is an integer which contradicts our assumption. Hence, there is no EF allocation exists.
% \end{proof}

% \begin{theorem}
% Given an arbitrary instance of \FISP/ with unit processing time jobs and cardinality weight, determining whether there is an EF allocation can be done in $O()$.
% \end{theorem}

% \begin{proof}
% Here, we prove the running time.
% \end{proof}

Now we consider the hardness of finding an EF allocation in the case in which each job has an unit processing time with a nonnegative weight, i.e., $\forall j\in\mathcal{J},p_j=1$ and $w_{ij}=w_j,\forall i\in[m]$.

\begin{theorem}
Given an arbitrary instance of \FISP/ with unit processing time job, it is NP-complete to determine whether there is an EF allocation or not.
\end{theorem}

\begin{proof}
We prove by give a polynomial reduction. We do reduction from the classical partition problem which is a well-known member of NP-complete class. In the partition problem, we are given a multiset $\mathcal{S}$ of positive integers, and the goal is to determine whether the multiset $\mathcal{S}$ can be partitioned into two subsets $\mathcal{S}_1$ and $\mathcal{S}_2$ such that the sum of the numbers in $\mathcal{S}_1$ equals the sum of the numbers in $\mathcal{S}_2$.

Given an arbitrary instance of partition problem, denoted by $PP$, we construct an instance of \FISP/ with unit processing time job as follows: for each element $e\in\mathcal{S}$, we create a job $j\in\mathcal{J}$ with the weight $e$. Moreover, each job has an unique time slot to process, i.e., $\forall j\in\mathcal{J},r_j+1=d_j$ and $\forall j,j'\in\mathcal{J},r_j\ne r_{j'}$. There are two agents included in the agent set, i.e., $\mathcal{A}=\set{a_1,a_2}$. Finally, we constructed an instance of \FISP/ with unit processing time jobs, denoted by $FIS$.

Now we consider the instance $PP$ and assume that there is a partition $\mathcal{S}=\mathcal{S}_1\cup\mathcal{S}_2$ such that $\sum_{e\in\mathcal{S}_1}e=\sum_{e'\in\mathcal{S}_2}e'$. It is easy to convert the partition $\set{\mathcal{S}_1,\mathcal{S}_2}$ to an EF allocation, denoted by $\mathcal{X}=\set{X_0,X_1,X_2}$, for corresponding \FISP/ instance $FIS$. Firstly, there is no job that assigned to charity, i.e., $X_0=\emptyset$. Then, we enumerate all the elements in $\mathcal{S}_1$ and $\mathcal{S}_2$ to construct $X_1$ and $X_2$, i.e., a job is assigned to agent $a_1$ ($a_2$) if and only if the corresponding element is in $\mathcal{S}_1$ ($\mathcal{S}_2$). Since all job has an unique time slot to process, there is feasibility problem which implies that the allocation $\mathcal{X}$ is a feasible allocation. Moreover, we have (i) $u_i(X_i)=u_i(X_i\cup X_0),\forall i\in\set{1,2}$ since $X_0=\emptyset$; (ii) $u_{1}(X_1)=u_{2}(X_2)$ since $\sum_{e\in\mathcal{S}_1}e=\sum_{e'\in\mathcal{S}_2}e'$. Therefore, $\mathcal{X}=\set{X_0,X_1,X_2}$ is an EF allocation.

Now we consider the instance $FIS$ and assume that there is an EF allocation, denoted by $\mathcal{X}=\set{X_0,X_1,X_2}$. Note that $X_0=\emptyset$ otherwise $u_1(X_1)<u_1(X_0\cup X_1)$ and $u_2(X_2)<u_2(X_0\cup X_2)$ which implies that $\mathcal{X}=\set{X_0,X_1,X_2}$ is not an EF allocation. Since $\mathcal{X}=\set{X_0,X_1,X_2}$ is an EF allocation, we have $u_1(X_1)=\sum_{j\in X_1}w_j \geqslant u_1(X_2)=\sum_{j\in X_2}w_j$ and $u_2(X_2)=\sum_{j\in X_2}w_j \geqslant u_2(X_1)=\sum_{j\in X_1}w_j$ which implies that $\sum_{j\in X_1}w_j = \sum_{j\in X_2}w_j$. Now we are ready to convert the EF allocation $\mathcal{X}=\set{X_0,X_1,X_2}$ to an partition, denoted by $\mathcal{S}=\set{\mathcal{S}_1,\mathcal{S}_2}$, for the partition instance $PP$. We enumerate all the jobs in $X_1$ and $X_2$ to construct $\mathcal{S}_1$ and $\mathcal{S}_2$, i.e., an element is added to $\mathcal{S}_1$ ($\mathcal{S}_2$) if and only if the corresponding job is in $X_1$ ($X_2$). Note that $X_0=\emptyset$. Since $\sum_{j\in X_1}w_j = \sum_{j\in X_2}w_j$, we find a partition such that the sum of the numbers in $\mathcal{S}_1$ equals the sum of the numbers in $\mathcal{S}_2$. 

Based on above polynomial reduction, a polynomial time algorithm, which can determine whether there is an EF allocation in the given instance of \FISP/, implies a polynomial time algorithm which can determine whether there is a desired partition in the corresponding instance of partition problem. Thus, P=NP which contradicts our assumption.

\end{proof}



==> 93-PO.tex <==
\section{EF1 versus PO}

In this section, we investigate the extent to which we can find an allocation that is both EF1 and PO.
we first show that EF1 and PO are actually not compatible even if agents' utilities are cardinality.
However, if all jobs further have unit processing time, then such an allocation exists and can be found in polynomial time. 

\begin{theorem}
EF1 and PO are not compatible for \FISP/ even if there are $m$ agents, for any $m\geqslant 2$, and agents have cardinality utilities. 
\label{thm:EF1_PO_noCompatible}
\end{theorem}

\begin{proof}
To prove \cref{thm:EF1_PO_noCompatible}, we show that any EF1 allocation for the instance in \cref{fig:EF1_PO_noCompatible} must not be a PO allocation. To show the above argument, we prove that any PO allocation must not be an EF1 allocation. We consider an arbitrary PO allocation, denoted by $\cX=\set{X_0,X_1,\cdots,X_m}$. We first prove that $\exists i\in[m]$ such that $X_i=\cJ_1$. We prove by contradiction and therefore assume that there is no $i\in[m]$ such that $X_i=\cJ_1$. Note that there must exist $i\in[m]$ such that $X_i\cap\cJ_1\ne\emptyset$ otherwise $\cX$ is not a PO allocation. Now we consider the job set, denoted by $X_l$, such that $X_l\cap\cJ_1\ne\emptyset$. Since every job in $\cJ_2$ overlaps with every job in $\cJ_1$, we have $X_l\cap\cJ_2=\emptyset$. Since $X_l\ne\cJ_1$, we can construct another feasible allocation $\cX'=\cX\cup\set{\cJ_1}\setminus X_l$. It is easy to see that $u_i(X_i') \geqslant u_i(X_i)$ for all $a_i\in\cA$ and $u_l(\cJ_1)>u_l(X_l)$ for agent $a_l$. This implies that $\cX$ is not a PO allocation.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=7cm]{Figures/EF1_PO_noCompatible.eps}
    \caption{The instance to show that the EF1 allocation is not compatible with PO allocation under the case where agents' utilities are cardinality, $p_j=d_j-r_j+1,\forall j\in\cJ$ and there are $m$ agents. The job set $\cJ=\cJ_1\cup\cJ_2$, where $\cJ_1=\set{j_1,j_2,j_3}$ and $\cJ_2=\set{j_4,j_5,\cdots,j_{m+2}}$. The agent set $\cA$ contains $m$ agents and $|\cJ|=|\cA|+2$. Each job $j\in\cJ_1$ has unit processing time and each job $j'\in\cJ_2$ has processing time 5.}
    \label{fig:EF1_PO_noCompatible}
\end{figure}

Therefore, we can assume that there must exist an $i\in[m]$ such that $X_i\in\cJ_1$. Without loss the generality, we assume that $X_1=\cJ_1$. Since $\cX$ is a PO allocation, we know that every remaining agent in $\cA\setminus\set{a_1}$ will receive exactly one job in $\cJ_2$. Without loss the generality, we assume that $X_i=\set{j_{i+2}}$. Therefore, we have $\cX=\set{X_0,X_1,\cdots,X_m}$, where $X_0=\emptyset,X_1=\cJ_1,X_2=\set{j_4},\cdots,X_m=\set{j_{m+2}}$. Since $u_i(X_1\setminus\set{j})=2>u_i(X_i)=1,\forall a_i\in\cA\setminus\set{a_1},\forall j\in X_1$, $\cX$ is not an EF1 allocation.
\end{proof}

\begin{theorem}\label{thm:EF1+PO:cardi}
A allocation that is simultaneously EF1 and PO exists and can be found in polynomial time if agents have cardinality utilities and all jobs have unit processing time.
\end{theorem}

Before we prove the Theorem \ref{thm:EF1+PO:cardi}, we first provide the following notations. Given an arbitrary instance of \FISP/ with unit processing time jobs and each agent has cardinality utility, for each job $j_i\in\cJ$, let $\mathcal{T}_i$ be the set of time slots included in the job window of $j_i$, i.e., $\mathcal{T}_i=\set{r_i,r_i+1,\cdots,d_i}$. Let $\mathcal{T}=\bigcup_{1\leqslant i \leqslant n}\mathcal{T}_i$. Note that the size of $\mathcal{T}$ can be bounded by $O(n^2)$, where $n$ is the number of jobs. For each each time slot $t_o\in\mathcal{T}$, we create $m$ copies, i.e., let $t_l^r$ be the $l$-th time slot in the $r$-th machine (agent), where $1\leqslant r \leqslant m$. Let $\mathcal{T}^M$ be the constructed time slot set. Note that the size of $\mathcal{T}^M$ can be bounded by $O(mn^2)$. Now we are ready to construct a bipartite graph $G(X\cup Y,E)$. For each job $j\in\mathcal{J}$, we have one vertex in $X$. For each time slot $t\in\mathcal{T}^M$, we have one vertex in $Y$. $E$ has an edge between a job vertex $x_i\in X$ and every time slot vertex in $\set{t_l^r|1\leqslant r \leqslant m}\subseteq \mathcal{T}^M$ if and only if $t_l\in\mathcal{T}_i$. In the reminder of this section, we define $G(X\cup Y,E)$ as $G(\mathcal{J},\mathcal{T})$ for convenience. Let $M$ be an arbitrary maximum matching in bipartite graph $G(\mathcal{J},\mathcal{T})$. Let $M(J)$ and $M(T)$ be the set of job vertices and time slot vertices in $M$, respectively. Let $\mathcal{J}_M$ be set of jobs whose corresponding job vertex is in $M(J)$, i.e., a job is included in $\mathcal{J}_M$ if and only if the corresponding job vertex is included in $M(J)$. Let $M_i\subseteq M$ be the set of (job, time slot) pairs whose time slot vertex is in $i$-th machine (agent), $1\leqslant i \leqslant m$, i.e., $M_i=\set{(j,t_l^r)\in M|r=i}$. Note that $\mathcal{M}=\set{M_1,M_2,\cdots,M_m}$ is a partition to $M$. Let $M_i(J)$ and $M_i(T)$ be the set of job vertices and time slot vertices included in matching $M_i$, respectively. Note that $\mathcal{M}(J)=\set{M_1(J),M_2(J),\cdots,M_m(J)}$ and $\mathcal{M}(T)=\set{M_1(T),M_2(T),\cdots,M_m(T)}$ is the partition to $M(J)$ and $M(T)$, respectively. Note that $|M_i|=|M_i(J)|=|M_i(T)|,\forall 1\leqslant i \leqslant m$.

\begin{algorithm}[htb]
\caption{\hspace{-2pt}{\bf .} Maximum matching-based algorithm for $p_j=1$ and cardinality utilities}
\label{alg:cardinality:p_j=1:EF1}
\begin{algorithmic}[1]
\REQUIRE $\mathcal{M}=\set{M_1,M_2,\cdots,M_m}$.
\ENSURE EF1 allocation $\mathcal{X}= (X_0, X_1, \cdots ,X_m)$.
\STATE $X_0=\mathcal{J}-\mathcal{J}_M$.
\WHILE{there is $M_i$ such that $|M_i|>\lceil \frac{|\mathcal{J}_M|}{m} \rceil$ or $|M_i| < \lfloor  \frac{|\mathcal{J}_M|}{m} \rfloor$}
\label{line:2}

\IF{$|M_i|>\lceil \frac{|\mathcal{J}_M|}{m} \rceil$}
    \WHILE{$|M_i|>\lceil \frac{|\mathcal{J}_M|}{m} \rceil$}
    \label{line:4}
        \STATE Find the $M_j=\min_{M_l\in\mathcal{M}}\{M_l\}$. 
        \STATE Find a pair $(j,t_l^i)\in M_i$ such that $t_l^j\notin M_j(T)$.
        \STATE $M_i=M_i\setminus\set{(j,t_l^i)}$.
        \STATE $M_j=M_j\cup\set{(j,t_l^j)}$.
    \ENDWHILE
    \label{line:9}
\ELSE
    \WHILE{$|M_i| < \lfloor  \frac{|\mathcal{J}_M|}{m} \rfloor$}
    \label{line:11}
        \STATE Find the $M_j=\max_{M_l\in\mathcal{M}}\{M_l\}$.
        \STATE Find a pair $(j,t_l^j)\in M_j$ such that $t_l^i\notin M_i(T)$.
        \STATE $M_i=M_i\cup\set{(j,t_l^i)}$.
        \STATE $M_j=M_j\setminus\set{(j,t_l^j)}$.
    \ENDWHILE
    \label{line:16}
\ENDIF

\ENDWHILE
\label{line:18}

\FOR{$1\leqslant i \leqslant m$}
    \STATE $X_i:=M_i(J)$.
\ENDFOR
\end{algorithmic}
\end{algorithm}

Let $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$ be the allocation returned by \cref{alg:cardinality:p_j=1:EF1}.

\begin{observation}
The allocation $\cX$ maximizes social welfare, i.e., there is no another feasible allocation $\cX'=\set{X_0',X_1',\cdots,X_m'}$ such that $\sum_{i=1}^{m}|X_i'|>\sum_{i=1}^{m}|X_i|$.
\label{obs:card:p_j=1:EF1:PO}
\end{observation}

\begin{lemma}
$u_i(X_i)\geqslant u_i(X_0\cup X_i),\forall 1\leqslant i \leqslant m$.
\label{lem:card:p_j=1:EF1:charity}
\end{lemma}

\begin{proof}
We prove by contradiction and therefore assume that there exist an agent $a_i\in\mathcal{A}$ such that $u_i(X_i) < u_i(X_0\cup X_i)$. We prove by constructing two bipartite graphs, denoted by $G(X_i,\mathcal{T}^1)$ and $G(X_0\cup X_i,\mathcal{T}^1)$. In $G(X_i,\mathcal{T}^1)$, we have $|X_i|$ vertices in one side, one vertex for one job in $X_i$, we have $|\mathcal{T}|$ vertices in another side, one vertex for one time slot in $\mathcal{T}$. There is an edge between job vertex and time slot vertex if and only if the time slot is in the job window. In $G(X_0\cup X_i,\mathcal{T}^1)$, we have $|X_0\cup X_i|$ vertices in one side, one vertex for one job in $X_0\cup X_i$, and the remaining part is similar as the $G(X_i,\mathcal{T}^1)$. Let $M_i,M_i'$ be the maximum matching in $G(X_i,\mathcal{T}^1),G(X_0\cup X_i,\mathcal{T}^1)$, respectively. Observe that $u_i(X_i)=|X_i|=|M_i|,u_i(X_0\cup X_i)=|M_i'|$ and therefore we have $|M_i|<|M_i'|$. Since the partition $\mathcal{M}=\set{M_1,\cdots,M_m}$ of the maximum matching in $G(\mathcal{J},\mathcal{T})$ corresponds to the allocation $\mathcal{X}=\set{X_0,X_1,\cdots,X_m}$ returned by \cref{alg:cardinality:p_j=1:EF1}, we construct a new  partition, denoted by $\mathcal{M}'$, in the following ways: $\mathcal{M}'=\mathcal{M}\cup\set{M_i'}\setminus\set{M_i}$. It is easy to see $\mathcal{M}'$ is a matching in $G(\mathcal{J},\mathcal{T})$. Since $|M_i|<|M_i'|$, we have $|\mathcal{M}'|=\sum_{M_i\in\mathcal{M}'}|M_i|>|\mathcal{M}|=\sum_{M_i\in\mathcal{M}}|M_i|$. This implies that $M$ is not the maximum matching in $G(\mathcal{J},\mathcal{T})$ which contradicts our assumption.
\end{proof}

\begin{lemma}
$u_i(X_i) \geqslant u_i(X_k\setminus\set{j}),\forall 1\leqslant i,k \leqslant m$ and $\exists j\in X_k$.
\label{lem:card:p_j=1:EF1:agents}
\end{lemma}

\begin{proof}
It is easy to see the correctness of \cref{lem:card:p_j=1:EF1:agents}. \cref{alg:cardinality:p_j=1:EF1} stops at case where there is no $X_i\in\mathcal{X}$ such that $|X_i|>\lceil \frac{|\mathcal{J}-X_0|}{m} \rceil$ or $|X_i|<\lfloor \frac{|\mathcal{J}-X_0|}{m} \rfloor$, which implies that $\forall X_i\in\mathcal{X},|X_i|\in\{\lceil \frac{|\mathcal{J}-X_0|}{m} \rceil ,  \lfloor \frac{|\mathcal{J}-X_0|}{m} \rfloor \}$. Therefore, we have $|X_i|-|X_k|\in\set{-1,0,1},\forall X_i,X_k\in\mathcal{X}$.
\end{proof}

Now we are ready to prove Theorem \ref{thm:EF1+PO:cardi}.

\begin{proof}[Proof of \cref{thm:EF1+PO:cardi}]
% According to \cref{lem:card:p_j=1:EF1:charity} and \cref{lem:card:p_j=1:EF1:agents}, we know that \cref{alg:cardinality:p_j=1:EF1} will returns an EF1 allocation.

According to \cref{obs:card:p_j=1:EF1:PO}, we know that the feasible allocation $\cX$ returned by \cref{alg:cardinality:p_j=1:EF1} maximizes the social welfare. Therefore, $\cX$ is a PO allocation. According to \cref{lem:card:p_j=1:EF1:charity}, we know that $\cX$ is an EF1 allocation. Hence, \cref{alg:cardinality:p_j=1:EF1} will returns a feasible allocation that is simultaneously EF1 and PO.

Now, we prove the running time. In each iteration, if there is a $M_i\in\mathcal{M}$ such that $|M_i|>\lceil \frac{|\mathcal{J}_M|}{m} \rceil$, then $\min_{M_k\in\mathcal{M}}\{|M_k|\} \leqslant \lfloor \frac{|\mathcal{J}_M|}{m} \rfloor$. If there is a $M_i\in\mathcal{M}$ such that $|M_i|<\lfloor \frac{|\mathcal{J}_M|}{m} \rfloor$, then $\max_{M_k\in\mathcal{M}}\{|M_k|\}\geqslant\lceil \frac{|\mathcal{J}_M|}{m} \rceil$. Therefore, it is impossible that if $|M_i|\in\{\lceil \frac{|\mathcal{J}_M||}{m} \rceil ,  \lfloor \frac{|\mathcal{J}_M||}{m} \rfloor \}$, $M_i\notin\{\lceil \frac{|\mathcal{J}_M||}{m} \rceil ,  \lfloor \frac{|\mathcal{J}_M||}{m} \rfloor \}$ again. This implies that line \ref{line:2}-\ref{line:18} of \cref{alg:cardinality:p_j=1:EF1} would be run at most $m$ times, where $m$ is the number of agents. Since there are $n$ jobs, line \ref{line:4}-\ref{line:9} (or line \ref{line:11}-\ref{line:16}) will be run at most $n$ times and each time requires the running time $O(m+n)$. Therefore, the running time of \cref{alg:cardinality:p_j=1:EF1} can be bounded by $O(mn\cdot(m+n))$. Since the number of vertices and edges of $G(\cJ,\cT)$ can be bounded by $O(mn^2)$ and $O(mn^3)$, finding the maximum matching requires $O(m^2n^5)$ by Hungarian Algorithm. Hence, given an arbitrary instance of \FISP/ with unit processing time and each agent has cardinality utility, the EF1 allocation can be found in $O(m^2n^5)$, where $m$ is the number agents and $n$ is the number of jobs. 
\end{proof}
